Sketch Video Synthesis

Understanding semantic intricacies and high-level concepts is essential in image sketch generation, and this challenge becomes even more formidable when applied to the domain of videos. To address this, we propose a novel optimization-based framework for sketching videos represented by the frame-wise B\'ezier curve. In detail, we first propose a cross-frame stroke initialization approach to warm up the location and the width of each curve. Then, we optimize the locations of these curves by utilizing a semantic loss based on CLIP features and a newly designed consistency loss using the self-decomposed 2D atlas network. Built upon these design elements, the resulting sketch video showcases impressive visual abstraction and temporal coherence. Furthermore, by transforming a video into SVG lines through the sketching process, our method unlocks applications in sketch-based video editing and video doodling, enabled through video composition, as exemplified in the teaser.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> method_backup.tex <==
% \input{figs/framework}
% \newpage
% page 3.5, end of related work
% \newpage
\input{figs/zero_shot_insight}
\section{Methods}

% We focus on xxx
% Define the task of style, foreground and background 

% How to achieve both precise localization and diverse editing effects? Different from existing optimization method (tune a video, text2live, shape-ware) zero-shot and short tuning
% (phylosophy of zero-shot editing, why it works?)



% our setting, from pretrained zero shot no need tuning for style and foreground. Tuning at object -level shape editing and large motion synthesis

% Define the setting of p2p2, notation. provide source, provide target

% Section overview and framework figures
We target zero-shot text-driven video editing~(\eg, style, attribute, and shape) without optimization for each editing prompt or the user-provided mask.
\RM{To edit a video, existing methods typically employ an optimization for editing prompt~\cite{shape-aware-editing, text2live} or source video~\cite{tuneavideo}, which is inconvenient and tedious in real applications. Besides, tuning a large model on a short video brings an additional trade-off between motion similarity and editing ability, where the model suffers from catastrophic forgetting after overfitting as in Fig.~\ref{fig:tuning progress}. }
% We find that simple text-based appearance editing, \eg, shape and local attribute editing, can be handled directly via the pretrained text-to-image model~\cite{stable-diffusion} by our new editing method. As for the challenge editing, \eg, shape-aware editing, our method can also gain better performance on the pre-trained one-shot video diffusion model~\cite{tuneavideo} than simple DDIM inversion~\cite{ddim}. 
Given a real video, we first invert it into a deterministic noise map as in Sec.~\ref{sec:invertibility_and_attention}. After that, we introduce our method that enables video editing  via network modification Sec.~\ref{sec:model} for appearance editing. Finally, we discuss a more challenging case that needs to edit the shape of the object in the video in Sec.~\ref{sec:shape-aware-editing}. The proposed method is a general editing method and can be used in various text-to-image or text-to-video models, in this paper, we majorly use Stable Diffusion~\cite{stable-diffusion} for its popularity and generalization ability.

% Below, we give the details of the basic information of DDIM inversion in Sec~\ref{sec:invertibility_and_attention}. Then, 
% we discuss our zero-shot editing method in Sec~\ref{sec:Attention during Inversion} and Sec~\ref{sec:Attention map mixing}.
% propose a general zero-shot video editing method that can be directly used for real video on the pre-trained models.
% Differently, we focus on zero-shot style and attribute video editing in our framework using the image diffusion model~\cite{stable-diffusion}, or shape editing using video model finetuned with shorter iteration (e.g., 100 iterations is enough for our results, while Tune-A-Video needs 300 to 500.). 


% \subsection{Spatial-temporal Model}

\RM{Since there is yet no publicly available video diffusion model, we build a backbone for our video editing problem.
To benefit from strong generative prior in pretrained model,
we extend the pretrained 2d U-Net from stable diffusion ~\cite{stable-diffusion} to a 3D temporal U-Net, following previous work~\cite{imagen-video, magic-video, tuneavideo}.
% In our implementation, for a $n,c,h,w$
Specifically, we add 1D temporal attention block and 1D low-rank~\cite{lora} temporal convolution after each 2D spatial convolution in the residual block. Besides, we inflate the self-attention layer to the spatial-temporal attention layer similar to Tune-a-video~\cite{tuneavideo}.
% to benefit from strong generative prior in pretrained model. 

Empirically, we find that inflating the deepest self-attention (channels $c=1280$, spatial resolution  $h\times w =8\times8$ ) 
and choose the frame in the middle (the third one for $n=8$ frames) as the key frame is sufficient for zero-shot style and attribute editing tasks. Formally, for latent $z^i$ at $\text{i}_{th}$ frame, we have $\text{Attention}(Q,K,V)$ as:
\vspace{-0.5em}
\begin{equation}
    Q=Q_s \mathbf{z}^i, K=K_s\left[\mathbf{z}_{n//2} ; \mathbf{z}_{i}\right], V=V_s\left[\mathbf{z}_{n//2} ; \mathbf{z}_{i}\right]
\end{equation}
As for video shape editing, inflating all self-attention to spatial-temporal attention with a one-shot tuning~\cite{tuneavideo} about 100 iterations brings much better results.


Inspired by the recent study of invertibility and attention reweight (Sec.~\ref{sec:invertibility_and_attention}) in diffusion models, we find the attention during inversion surprisingly suitable for structure and semantic control for images and videos~(Sec.~\ref{Attention during Inversion}). To further improve the shape editing quality of our model, we adopt the one-shot tuning strategy~\cite{tuneavideo} and a novel Self-attention mixing strategy~(Sec.~\ref{sec:Attention map mixing}). Finally, we analyze the temporal consistency property of our method \chenyang{How to analyze}}




\label{sec:method}



% \subsection{Framework overview}
% \subsection{Real Image Inverting and attention Editing}
\subsection{Video Inversion using DDIM Inversion}
\label{sec:invertibility_and_attention}
Recently, Latent Diffusion Models~\cite{stable-diffusion} are introduced to diffuse and denoise the latent space of an autoencoder. Firstly, an encoder $\mathcal{E}$ compresses an RGB image $x$ to a low-resolution latent $\mathcal{E}(x)=z$, such that the latent can be reconstructed back by decoder $\mathcal{D}$ to image $\mathcal{D}(z) \approx x$. Secondly, a U-Net $\varepsilon_\theta$ composed of cross-attention and self-attention ~\cite{attention_is_all_you_need} is trained to remove the artificial noise using the objective:
\vspace{-0.5em}
\begin{equation}
\min _\theta E_{z_0, \varepsilon \sim N(0, I), t \sim \text { Uniform }(1, T)}\left\|\varepsilon-\varepsilon_\theta\left(z_t, t, p \right)\right\|_2^2,
\end{equation}
% \vspace{-0.2em}
where $p$ is the embedding of the conditional text prompt and $z_t$ is a noised sample of $z_0$ with noise of random sampled timestep $t$.

During inference, deterministic DDIM sampling~\cite{ddim} is employed to convert a random noise $z_T$ to a clean latent $z_0$ in a sequence of timestep $t\in[0, T-1]$: 
\vspace{-0.5em}
\begin{equation}
    z_{t-1} = \sqrt{\alpha_{t-1}} \; \frac{z_t - \sqrt{1-\alpha_t}{\varepsilon_\theta}}{\sqrt{\alpha_t}}+ \sqrt{1-\alpha_{t-1}}{\varepsilon_\theta},
\end{equation}
\label{eq: denoise}
where $\alpha_{t}$ are parameters for noise scheduling~\cite{ddim, ddpm}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/imgs/methods/method_inversion_recons_attention-cropped.pdf}
    \caption{\textbf{Zero-shot local attributed editing (cat $\rightarrow$ tiger) using stable diffusion.} Inversion-time cross-attention provides more accurate structure guidance and editing ability than reconstruction-time cross-attention. \xiaodong{add a,b to the two figure} }
    \label{fig:attention comparison}
\end{figure}

Based on the ODE limit analysis of diffusion process, DDIM inversion~\cite{ddim,DiffusionBeatGANs} is proposed to map a clean latent $z_0$ back to a noised latent $\hat{z}_T$ in revered steps:
\begin{equation}
    \hat{z}_{t+1} = \sqrt{\alpha_{t+1}} \; \frac{\hat{z}_t - \sqrt{1-\alpha_t}{\varepsilon_\theta}}{\sqrt{\alpha_t}}+ \sqrt{1-\alpha_{t+1}}{\varepsilon_\theta}.
\end{equation}
\label{eq: add noise}
Such that the inverted latent $\hat{z}_T$ can reconstruct an latent $\text{DDIM}(\hat{z}_T) \approx z_0$ similar to the clean latent $z_0$ at classifier-free guidance scale $s_{cfg} = 1$.
To improve the generation quality, recent methods use a large classifier-free guidance scale $s_{cfg} \gg 1$. 

\RM{However, as shown in the DDIM reconstruction of Fig.~\ref{fig:attention comparison}~(a), a naive DDIM inversion and reconstruction with $s_{cfg} \gg 1$ lose the layout (mirrors) and inner structure (cat) of objects in the image.

To constrain the structure of the generated image, Prompt2Prompt~\cite{p2p}
% replaces the cross-attention maps of U-Net $\varepsilon_\theta$ during the editing with the maps stored during the reconstructed time. 
edits the cross-attention maps of U-Net $\varepsilon_\theta$ during editing. 

More Formally, for each cross-attention block, the attention maps of the input spatial features $\phi(z_t)$ are
% are projected into a query matrix $Q_c(\phi(z_t)$ and key $K_c(p_{edit})$ matrics
% the attention maps are
\begin{equation}
    M_c=\operatorname{Softmax}\left(\frac{Q_c(\phi(z_t)) K_c(p)^T}{\sqrt{d}}\right),
\end{equation}
where $Q_c(\phi(z_t))$ is the query matrix of spatial features, $K_c(p_{edit})$ is the key matrix of prompt $p$. During editing, Replacing the maps $M_c(p_{edit})$ with those from reconstruction $M_c(p_{src})$ results in an edited image, which has a similar semantic layout as the reconstructed one, as shown in the Fig.~\ref{fig:attention comparison}~(a). }

\subsection{Attention during Inversion}
\label{sec:Attention during Inversion}

Although the attention maps during reconstruction have been utilized~\cite{p2p, pnp, pix2pix-zero} to control the semantic layout of the generated images, an efficient and high-quality source image reconstruction without any optimization is still a challenge. The problem comes from two folds. First, the invertible property of DDIM discussed in Eq.~\eqref{eq: denoise} and Eq.~\eqref{eq: add noise} only holds in the limit of small steps. However, current methods set the step as 50 to accelerate the pipeline, which brings an accumulation of errors in each time step. Secondly, a large classifier-free guidance $s_{cfg} \gg 1$ also brings inconsistency between inversion and editing, while a small $s_{cfg} = 1$ does not have enough editing ability. Therefore, previous methods requires optimization of text-embedding ~\cite{p2p} or other regularization~\cite{pix2pix-zero}.

In contrast with previous methods, our framework utilizes the attention maps during inversion steps (Eq.~\eqref{eq: add noise}), which is available because the source prompt $p_{src}$ and initial latent $\mathcal{E}(x) = z_0$ are provided to the U-Net $\varepsilon_\theta$ during inversion. As observed in the bottom part of Fig.~\ref{fig:attention comparison}, the cross-attention map during inversion captures the silhouette and the pose of the cat in the source image, while the map during reconstruction has a noticeable difference. The gap between inversion and reconstruction is more severe in zero-shot video editing as shown in the Fig.~\ref{fig:ablation_video_inversion_attn}, since there is yet no video diffusion model available for high quality inversion.

Formally, during inversion, we derive the final latents representations and attention maps from the video at each denoising timestep $t$ as:
\begin{equation}
z_T, [c_{t}^{\text{src}}]_{t=1}^T, [s_{t}^{\text{src}}]_{t=1}^T=\Call{DDIMInv}{z_0, p_{src}},
\end{equation}
where latents $z_T$ has a shape of $n\times c \times h \times w  = 8\times4\times64\times64$ in our implementation. 
Cross attention maps $c_t^{src}$ has the shape of  
$ \text{frames}  \times \text{attention\_head} \times \text{pixels} \times \text{text\_token}  = 8\times8\times\{hw\}\times77$, which is correspondence between each pixel and each word token.
Similarly, self-attention maps have the shape of  $ \text{frames}  \times \text{attention\_head} \times \text{pixels} \times \text{pixels} \}  = 8\times8\times\{hw\}\times\{hw\}$, which represent the inner structure in each frame and implicit warping between frames  at different temporal index.

During the editing stage, we predict the noise to remove by fusion the attention from inversion: 
\begin{equation}
\hat{\epsilon}_t = \Call{AttenFusionUNet}{\theta, z_t, t, p_{\text{edit}},c_{t}^{\text{src}}, s_{t}^{\text{src}}}
\end{equation}

Fig.~\ref{fig:attention comparison} presents a visualization of our attention fusion between inversion and editing. The bottom part replaces the full-resolution cross-attention and self-attention maps following prompt-to-prompt~\cite{p2p}. The result shows that the texture and color attribute of the input image is successfully edited to the target prompt without changing the pose and background details. Compared with the result from reconstruction attention injection and optimization-based image editing method~\cite{null}, our inversion attention injection builds a strong zero-shot editing method.
% ablation study show that xxx
% ~\ref{ablation:}


% \newpage

\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{figs/imgs/methods/method_self_atten_mask-cropped.pdf}
    \caption{\textbf{Zero-shot shape editing (rabbit $\rightarrow$ tiger) using stable diffusion}. Right column: It is difficult to find a naive timestep replacement percentage for self-attention. Left: If we mask the self-attention using the cross-attention map obtained during inversion, the editing result has both new target shape from text with similar pose and background from input frame.}
    \label{fig: attention mixing}
\end{figure}

\subsection{Attention Map Fusion}
\label{sec:Attention map mixing}
Existing attention fusion methods~\cite{p2p,null} replace full-resolution cross-attention maps ($(hw) \times (token_num)$) and self-attention maps $(hw) \times (hw)$ to preserve the background and object structure in the source image, which is presented in Fig.~\ref{fig:attention comparison}.
% shows that this full-resolution fusion edits the attribute without changing the pose structure.
However, this strategy can be insufficient in object shape editing, as shown in an image example in Fig.~\ref{fig: attention mixing}. In the third column, replacing self-attention $s^{edit} \in \mathbb{R}^{hw \times hw} $ with $s^{src}$ brings unnecessary structure leakage and the generated image has unpleasant blending artifacts in the visualization. On the other hand, if we keep $s^{edit}$ during DDIM denoising pipeline, the structure of the background and watermelon have unwanted changes and the pose of the original rabbit is also lost. Inspired by the fact that the cross-attention map during inversion provides the semantic layout of the input image (the second rows in Fig.~\ref{fig: attention mixing}), we propose to first obtain a binary mask by thresholding the cross-attention map during inversion, then blend the self-attention maps of editing and inversion stage with the binary mask, as illustrated in Fig.~\ref{fig:main_framework}. Formally, the attetnion map fusion is implemented as 
\begin{equation}
M = \Call{Heavisidestep(c_t^{src})}{}
\end{equation}




% 3. what solution we choose: mask the self attention in low resolution layer 8X8, 16X16 using layout of cross attention



4. what is our implementation
write the math formation


\subsection{Analysis of Temporal Consistency}

1. tune-a-video spatial-temporal attention
2. Motion , representation
3. 


% \newpage




% \input{algs/alg_main}

% \newpage



\subsection{Application as zero-shot image editing}

page 5
% \newpage

